SoundSieve: Seconds-Long Audio Event Recognition on Intermittently-Powered Systems

A fundamental problem of every intermittently-powered sensing system is that signals acquired by these systems over a longer period in time are also intermittent. As a consequence, these systems fail to capture parts of a longer-duration event that spans over multiple charge-discharge cycles of the capacitor that stores the harvested energy. From an application's perspective, this is viewed as sporadic bursts of missing values in the input data -- which may not be recoverable using statistical interpolation or imputation methods. In this paper, we study this problem in the light of an intermittent audio classification system and design an end-to-end system -- SoundSieve -- that is capable of accurately classifying audio events that span multiple on-off cycles of the intermittent system. SoundSieve employs an offline audio analyzer that learns to identify and predict important segments of an audio clip that must be sampled to ensure accurate classification of the audio. At runtime, SoundSieve employs a lightweight, energy- and content-aware audio sampler that decides when the system should wake up to capture the next chunk of audio; and a lightweight, intermittence-aware audio classifier that performs imputation and on-device inference. Through extensive evaluations using popular audio datasets as well as real systems, we demonstrate that SoundSieve yields 5%--30% more accurate inference results than the state-of-the-art.

==> tex/02_study.tex <==

\section{Empirical Study}

%Signals acquired by intermittent systems over a long period in time are intermittent. To the application, this manifests as sporadic bursts of missing values in the input data -- which may or may not be recoverable using statistical or data-driven methods. Prior to designing \sys, we conduct studies to understand how severe this problem is and explore possible solutions.   

In order to understand the effect of missing values caused by intermittence, we conduct an empirical study on three popular audio datasets: Urban8K~\cite{urban}, ESC-50~\cite{piczak2015esc}, and GSC~\cite{warden2018speech}. These datasets contain over 115,000 audio clips of over 95 different categories.

\subsection{Dealing With Missing Values}

%\parlabel{Effect of Missing Samples.} 

A classifier that does not explicitly handle missing values performs extremely poorly when it encounters such inputs. This is evident in Figure~\ref{fig:iasa} -- confirming similar prior studies~\cite{perforation} -- where we see 20\%--50\% drop in inference accuracy (referred to as \emph{do nothing}) when $75\%$ of the data are missing. 

\begin{figure}[!htb]
    \centering
    \vspace{-5pt}
    \includegraphics[width=0.75\linewidth]{tex/figs/figure_2.pdf}
    \caption{Imputation and augmentation increase accuracy, but cannot maximize the gain in accuracy by themselves. The percentage of missing values in the experiment is $75\%$.}
    %\rnote{new plot}}
    \label{fig:iasa}
\end{figure}

To address this issue, there are two generic classes of solutions in the literature: (a) estimating (imputing) the missing values (before classification) using statistical or neural methods, and (b) training the classifier on an augmented dataset where missing values are synthetically introduced in the training examples. Although implementing any or both of these techniques improve the classification accuracy -- referred to as \emph{imputation} and \emph{augmentation}, respectively --  there is still a large gap of 5\%--40\% in accuracy that cannot be regained. Furthermore, the classifier used in this experiment is a state-of-the-art CNN having 1008 filters, which is not feasible for intermittent systems. In conclusion, \textbf{data imputation and/or data augmentation cannot completely solve the intermittent audio classification problem. We need to complement them with audio content-aware intelligent sampling at the front to maximize their performance.}       



%\parlabel{Feasibility of Content-Aware Sampling.} 

%\vspace{-10pt}
\subsection{Feasibility of Content-Aware Sampling}

Although an intermittent system does not have complete control over the harvesting (charging) cycles, which depend on the energy source, once charged, the system can decide when to use that harvested energy. This creates an opportunity for the system to selectively sample segments of the audio that are more informative and relevant to audio classification. 

We conduct another study to understand what percentage of an audio clip must be sampled so that we have enough information to classify a clip correctly. To conduct this study, we (logically) divide each clip into non-overlapping 100ms \emph{segments} and  search for the smallest set of \emph{K} most informative segments that must be sampled to correctly classify the clip. We keep the \emph{K} selected segments intact, and impute the rest of the segments prior to classifying the clip. The outcome of this experiment is summarized in Table~\ref{table:cumulative_importance}.        

%Car horn, siren; Music; Dog bark; Drilling, jackhammer; children playing; brushing; Breathing, snoring; Coughing, sneezing; animal; Can opening, glass breaking; Drinking, sipping; Flushing, washing machine;    

\begin{table} [!htb]
\vspace{-5pt}
\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{|l|l|rrrrr|} 
%\hline
\hline
\textbf{Sound Category} & \textbf{\#Clips} & \textbf{K=10\%}  & \textbf{K=30\%} & \textbf{K=50\%} & \textbf{K=70\%} & \textbf{K=90\%}
\\
\hline
\textbf{Voice Command} & 600 & 64.20\% & 81.50\% & 88.70\%  & 100.00\% & 100.00\%
\\
\textbf{Vibration} & 120 & 56.62\% & 81.18\% & 92.31\% & 93.47\% & 94.20\%
\\
\textbf{Alarm} & 85 & 54.62\% & 85.09\% & 91.91\% & 93.11\% & 93.50\%
\\
\textbf{Children} & 80 & 56.62\% & 88.82\% & 92.19\% & 94.61\% & 95.95\%
\\
\textbf{Music} & 76 & 48.52\% & 82.29\% & 89.61\% & 91.47\% & 94.14\%
\\
\textbf{Pet} & 76 & 52.27\% & 83.61\% & 92.10\% & 94.27\% & 95.10\%
\\
\textbf{Animal} & 65 & 54.68\% & 90.63\% & 92.21\% & 93.00\% & 100.00\%
\\
\textbf{Bursts} & 16  & 51.13\% & 65.90\% & 81.81\% & 85.20\% & 92.00\% 
\\
\textbf{Laundry} & 16  & 54.10\% & 69.70\% & 83.10\% & 89.40\% & 98.00\% 
\\
\textbf{Sleep} & 16  & 56.21\% & 72.27\% & 80.53\% & 88.96\% & 100.00\%
\\
\textbf{Wellness} & 16  & 64.32\% & 85.42\% & 88.78\% & 100.00\% & 100.00\%
\\
\textbf{Bathroom} & 12  & 61.11\% & 83.33\% & 90.00\% & 100.00\% & 100.00\%
\\
\textbf{Drink} & 12  & 55.32\% & 67.40\% & 84.18\% & 86.24\% & 95.00\% 
\\
\hline
\textbf{Overall} & 1190 & 51.47\% & 85.91\% & 89.60\%  & 92.30\% & 96.60\%
\\

\hline
%\textbf{GTSRB}~\cite{stallkamp2011german} & -\% & -\% & -\% & -\% & -\% 
%\\
%\textbf{AlexNet}~\cite{krizhevsky2012imagenet} (\textbf{UrbanSound8K}~\cite{su2019environment}) & -\% & -\% & -\% & -\% & -\%
%\\
\end{tabular}
%\captionsetup{font=normalsize}
\captionsetup{font=Large}
\caption{The percentage of clips that are classified correctly when we sample \emph{K\%} most informative segments.}
\label{table:cumulative_importance}
\begin{tablenotes}[para,flushleft]
    %* table note
\end{tablenotes}
\end{threeparttable}
}
\vspace{-13pt}
\end{table}

Each row of Table~\ref{table:cumulative_importance} is a cumulative distribution of \emph{K} for a certain audio category, where \emph{K} denotes the minimum number of most informative segments to sample to classify an audio correctly. For example, the last number of the first row tells us -- if we sample the most informative 90\% segments (and impute the remaining 10\%), we can correctly classify 93.5\% of the alarm sounds from Urban8k dataset. Figure~\ref{fig:CDFs} shows the same information as in Table~\ref{table:cumulative_importance} but separately for each dataset.      

\begin{figure}[!thb]
  \centering
  \begin{subfigure}[b]{0.225\textwidth}
    \includegraphics[width=\textwidth]{tex/figs/motivation_1_Urban.png}
    \caption{Urban8k}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.225\textwidth}
    \includegraphics[width=\textwidth]{tex/figs/motivation_1_ESC_indoor.png}
    \caption{ESC-indoor}
  \end{subfigure}
  \\
  \begin{subfigure}[b]{0.225\textwidth}
    \includegraphics[width=\textwidth]{tex/figs/motivation_1_ESC_animal.png}
    \caption{ESC-animal}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.225\textwidth}
    \includegraphics[width=\textwidth]{tex/figs/motivation_1_GSC.png}
    \caption{GSC}
  \end{subfigure}
  \caption{The distribution of correctly-classified clips in each dataset when \emph{K} most informative segments are sampled.}
  \vspace{-5pt}
  \label{fig:CDFs}
\end{figure}

This result provides insights into the redundancy in audio clips for classification purposes. For an intermittent system, from its charge and discharge times, we can estimate what fraction of the time the system can sample, and then estimate their expected inference accuracy from these distributions. These datasets, however, are trimmed and preprocessed to remove unwanted sounds. In real-world audio, we expect more redundancy and thus an intermittent system is expected to have more room for selecting informative segments to achieve higher accuracy than the estimated values in this study. In conclusion, \textbf{not all audio segments being equally informative, a content-aware sampler on a resource-constrained sensing system can select a subset of informative audio segments to maximize their ability to correctly classify long-duration audio clips.}   

\subsection{Sparsity of Audio Events}

In order to classify audio events on an intermittent system, one may choose to use a very large capacitor to ensure that the system never goes out of energy while sensing an event. Large capacitors, however, take longer time to charge, and when the gap between two consecutive audio events is shorter than the charging time of the capacitor, the system will miss audio events.

\begin{figure}[!htb]
    \centering
    \vspace{-5pt}
    \includegraphics[width=0.9\linewidth]{tex/figs/motivation_1.pdf}
    \caption{Percentage of audio events that are missed for different capacitor sizes at different energy harvesting rates. C denotes the ratio between charging and discharging times of the capacitor.}
    %\rnote{new plot}}
    \label{fig:motivation_1}
\end{figure}

We conduct an experiment to quantify the number of missed audio events for different sizes of the capacitor and energy harvesting rates. We use the DCASE SELD dataset~\cite{DCASE_SELD} which contains over 600 audio scenes of 60 seconds length recorded in a wide variety of environments such as modern classrooms, meeting rooms, large cafeterias, and open gym spaces. These recordings contain real-world background noises such as ventilation noise and people chatting. We vary the size of the capacitor~(from $100 \mu F$ to $10$ mF) and the energy harvesting parameter, $C$ (from 1 to 3), and from the charging and discharging times of the capacitor, we quantify what fraction of the audio events are missed (completely) by a typical intermittent system.

Figure~\ref{fig:motivation_1} shows that with larger capacitors, e.g., $10mF$, as many as 70\% of the audio events are missed in real-world scenarios. In contrast, smaller capacitors, e.g., $100\mu F$, results in as low as 4\% missed audio events, but the captured audio events have many missing samples or holes in them -- which calls for an intelligent audio sampling and processing technique that can deal with missing samples in intermittent audio sensing systems.

%This is different than information theoretic bounds on sampling which are for complete reconstruction of the signal. 





==> tex/03_overview.tex <==
% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=\textwidth]{tex/figs/overview.pdf}
%     \caption{System overview}
%     \label{fig:overview}
% \end{figure*}

\begin{figure*}[!thb] 
    \centering
    \subfloat[Offline Phase]{
        \includegraphics[width=0.5\textwidth]{tex/figs/overview_offline.pdf} 
    }
    \subfloat[Online Phase]{
        \includegraphics[width = 0.5\textwidth]{tex/figs/overview_online.pdf}     
    }
    \caption{\sys consists of two phases: (a) an offline phase for audio analysis and modeling, and (b) an online (real-time) phase for audio sensing and inference on an intermittent system. }
    \label{fig:overview}
\end{figure*} 

%\newpage

\section{Overview of \SYS}

\sys is an audio sensing and inference framework that enables seconds-long audio event recognition on intermittently-powered systems. At the heart of \sys is a lightweight, content-aware sampling algorithm that decides (in real-time) when the system should wake up from sleep to actively sample the next few segments of the incoming audio. \sys's sampling objective is to maximize the classification accuracy by capturing the most informative audio segments, given the remaining charge in the capacitor, which limits the maximum number of segments the system can sample before it runs out of harvested energy.  

\sys is a software-only solution which does not require specialized hardware or multiple collaborating nodes. The framework consists of two phases: (a) an offline phase for audio analysis and modeling, and (b) an online (real-time) phase for audio sensing and inference on an intermittent system. Figure~\ref{fig:overview} shows both phases along with the major processing steps in them.                  

%The system is generalized enough to work with different kinds of classification models and audio events. It only requires a pre-trained classifier and training dataset to analyze and prepare a audio sampler that can sample and process audio in real-world intermittent systems. 

%There are four major components in our SoundSieve system- audio imputation, classification network, the block importance analyzer, and the audio sampler. 

\subsection{Audio Analysis and Modeling}

\parlabel{Audio Segment Importance.} \sys logically divides audio clips into non-overlapping 100ms \emph{segments}, and processes one segment at a time. Each audio segment is assigned an importance score that denotes how important that segment is for accurate classification of the clip. During the offline phase of \sys, the importance score of each 100ms segment of every audio clip in the dataset is computed.     

%This higher the value is, the more important that audio segment is . A negative score corresponds to a negative correlation between that audio block and the classification accuracy.

%\parlabel{Perforation Mask.} While computing the block importance score, we augment each audio signal by randomly introducing perforation in them. If there are total $n$ audio blocks, we create a perforation mask of length $n$. If the $i$-th value of the perforation mask is zero, we assume there is no audio signal present in that time. We perform this augmentation for each audio signal in training data. Then we use audio imputation in the frequency domain to impute the missing segments and feed them in our pre-trained classifier. This provides us the model prediction which we use to compute the importance of each audio block.



\parlabel{Predicting Segment Importance Scores.} In order for \sys to decide which segments to capture next, the system must be able to predict the importance of the next few segments in the incoming audio. To enable this, during the offline phase of \sys, a simple regression network (which runs on the intermittent platform in real-time) is trained. The predictor predicts the importance score of up to 10 next segments, given the frequency domain features of the audio segment that has just been read.          


%We train a simple regression network to estimate the importance of next $n$ audio blocks given the frequency domain information at current time. This provides us a probabilistic estimation of information that can be gained from next $n$ blocks of audio. We also use an aggregation of the importance of each audio block in each training data to generate a global importance of each block and use them in combination with local importance values. The regression network is trained offline and used to estimate importance in real-world intermittent system. 

\subsection{Audio Sensing and Inference}

\parlabel{Sampling.} \sys's audio processing system is triggered by the microphone, which remains in ultra-low-power listening mode and sends an interrupt to the microcontroller whenever a sound is detected. \sys reads an audio segment and extracts its spectral features. The sampling controller uses these features and the offline-trained importance predictor to identify potential candidate segments to read, and based on the remaining charge in the energy buffer, it decides whether (and for how long) it should go into to the low-power mode before it samples the next segment.        

%to predict the importance scores of the incoming segments and based on the both the   using the offline-trained segment imporatance predictor   

%We use the estimated importance score from regression network and current energy level of the energy buffer to decide how long the system should go into low-power mode before starting sensing again. If the energy buffer is full and the next most informative block is further away in time domain, then the system decides to sense the next most informative block. Thus the system takes the energy availability into account while deciding to sense more informative blocks.

%\subsection{Audio Classifier}

\parlabel{Imputation.} Once the audio event ends, prior to classifying, the missing segments in the sampled audio are imputed to estimate the missing values. A lightweight, hierarchical interpolation technique is used to impute the missing audio segments. 

%Due to energy availability, an intermittent system can be in low-power mode for varying amount of time. After the audio event finishes, we take each segment of missing audio and impute them in the frequency domain using the frequency domain information at the time immediately before and after the missing segment.

\parlabel{Classification.} An offline-trained convolutional neural network (CNN) is used to classify the audio. The classifier is trained on an augmented dataset where missing values are synthetically introduced at random locations in the audio clip and then the audio is imputed. To be able to classify audio signals of arbitrary lengths, a global max pooling layer is used after the final convolution layer, and only one value from each channel is fed to the fully connected layer.               

%consists of convolution and fully connected layers for each audio events. During training of the network, we use both clean audio signal and augmented audio signal where we randomly create missing audio segments in the audio signal and impute them using our audio imputation method. We also use a global max pooling layer after the final convolution layer and feed only one value from each channel to the fully connected layer. This makes the network robust enough to handle audio signal of arbitrary length.


\begin{comment}
The general idea of our offline computation is to analyze training data before real-time deployment of an intermittent sensing system and generate a light-weight scheme that can be used to schedule sensing while maximizing classification accuracy. Due to the limitation of energy harvesting and capacitor, an intermittent system must go through a cycle of charging and discharging and only during discharging the system can execute tasks. That is why we need to identify a method that can assist a real-time scheduler to determine when it would be optimal to go for charging the capacitor by analyzing training data.

In order to achieve this goal, we divide the audio signal that needs to be classified into blocks of audio segment where each block has a length of $t_{block}$ seconds. After sensing audio for $t_{block}$ seconds, we need to determine via a scheduling method when it would be most optimal to sense again in real-time. However if the execution algorithms consumes more energy than sensing continuously, it defeats the purpose of scheduling. That is why we decided to couple the data processing and the scheduling algorithm with the classification algorithm. 

Our system processes the audio data for a fixed window length and performs data processing such as fast Fourier transform~(MFCC) to compute the frequency domain information. Then we feed this processed data to a RNN encoder to compute the hidden state output. Note that during processing of each audio window, we retain the internal state of the RNN and hence the hidden state we compute at time step, $t_i$ retains information of all previous time steps. Then this hiddent state value is fed into a fully connected network that predicts the importance of next $n$ blocks. This lightweight model is trained offline by analyzing the training data. We first train an end-to-end DNN to classify an audio event. Then we use local interpretable model-agnostic explanation to compute the importance of each time step of certain window length in classification process. Then we train the FC layer that takes the current hidden layer output of the RNN layer and current time-step value and predicts the importance of next $n$ blocks.
Finally in real time, we analyze the probabilistic importance of next $n$ blocks and current energy level to decide how long should the MCU stay in low-power mode and harvest energy before going into active mode again to sense the audio signal that will contain the most information to classify the corresponding audio event.
\end{comment}


==> tex/temp/04_encoder.tex <==
\section{Audio Analyzer}

The goal of the block importance analyzer is to analyze the pre-trained classification network and compute importance of blocks of audio segment when predicting an audio event. Next we train an extremely lightweight Gaussian process regressor to predict the importance of future blocks according to the observed audio signal at current time-step.

\subsection{Block Importance Computation}
After we train our classifier network, we move to identify which block of audio are most informative in terms of providing an accurate prediction. We use the a technique similar to the local interpretable model agnostic explanation~(LIME)~\cite{} of each data point to compute this importance.

In LIME, a local explanation is depicted as a model, $g\in G$ where $G$ can be any simple and interpretable model such as linear models. The interpretable model $g$ has a domain of $\{0,1\}^{d'}$, representing either the presence or absence of a feature. In our algorithm, we select audio segment of length $\Delta t$ as feature that are randomly turned on or off to create augmented datapoints, $z$ from the original datapoint, $x$. However, we use the imputation in the frequency domain instead of feeding zero values directly. Since we use audio imputaion during real-time inference anyway, we identify which blocks can lead to drop in classification accuracy even after the imputation.

Next we feed the augmented datapoints to the original classifier, $f$ and compute the prediction values. Then we train a simple linear ridge regressor, $g$ that minimizes the measurement of how unfaithful $g$ is in approximating $f$ in the locality defined by the cosine distance metric. The goal of the linear regressor is to minimize the following loss function:

\begin{equation}
    \epsilon(x) = argmin_{g\in G} L(f,g,\Pi_x)
\end{equation}

Here, $L(f,g,\Pi_x)$ is the measurement of how $g$ approximates the original classifier $f$. 

\subsection{Block Importance Prediction}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.5\textwidth]{tex/figs/importance.PNG}
    \caption{Next n-block importance predictor}
    \label{fig:importance}
\end{figure}

We compute this local explanation for each datapoint, while storing the internal states of RNN for future use.  After explanation of all datapoints are computed, we move towards computing an approximate model to predict the importance of sensing audio from time step $t_i$ to $t_{i+n}$, given that we already observed or skipped the audio signal upto time-step $t_{i-1}$. For example, suppose during the datapoint augmentation while training the simple interpretable model, we read the first audio segment, then skip the audio segment at time-step 1 and then read the audio from next segment again and so on. Given that we already know the importance of each time-step for classification accuracy, we train a simple neural network that takes the last hidden state output of the RNN and current time-step as input and predicts the importance of next $n$ audio segments of length $\Delta t$. This predictions, although not fully accurate, can work as a guideline to decide which audio segments are most important and maximizes the classification accuracy. A brief overview of the algorithm for calculating importance is given in algorithm~\ref{algo:importance}.

From this analysis of training data, we get a historical estimate of how much next $n$ blocks may contribute toward classification of current audio clip, given the observed signal upto that time-step. We save the trained audio classification model and the importance prediction model to utilize when doing real-time inference in an intermittent system.

\begin{algorithm}
\caption{Audio Importance Calculation}
\label{algo:importance}
\begin{algorithmic}[1]
\Require Audio feature $X$, Ground truth $Y$, Trained Classifier $f$, Length of each audio window $K$, Number of augmentation $n_{aug}$, Importance prediction length $n$

\State $E\gets \{\}$
\For{$k\in length(X)$}
    \State $x, y = X_k, Y_k$
    \State $Z\gets \{\}$
    \For{$i\in\{1,2, ... n_{aug}\}$}
        \State $z_i, mask_i\gets Segment(x, K)$
        \State $pred_i, hidden_i \gets f(z_i)$
        \If{$pred_i= y$}
            \State $Z\gets Z \cup (z_i, pred_i, hidden_i)$
        \EndIf
    \EndFor
    \State $explanation_k \gets Ridge Regression(Z)$
    \State $E\gets E\cup (explanation_k, Z_k[hidden])$
\EndFor
\State $X_{imp}, Y_{imp}\gets \{\}$
\For{$k\in length(X)$}
    \For{$i\in \{1,2,...,N\}$}
        \State $e_k, h_k\gets E_k$
        \State $t_{ik}\gets Random(0, length(X_k)-t_n)$
        \State $X_{imp}\gets X_{imp}\cup (h_k[0:t_{ik}], t_{ik})$
        \State $Y_{imp}\gets Y_{imp}\cup (e_k[t_{ik+1}:t_{ik+n}])$
    \EndFor
\EndFor
\State  $IP \gets Train(X_{imp}, Y_{imp})$
\newline
\Return IP
\end{algorithmic}
\end{algorithm}









==> tex/temp/04_offline_scheduling.tex <==
\section{Offline computation}

The general idea of our offline computation is to analyze training data before real-time deployment of an intermittent sensing system and generate a light-weight scheme that can be used to schedule sensing while maximizing classification accuracy. Due to the limitation of energy harvesting and capacitor, an intermittent system must go through a cycle of charging and discharging and only during discharging the system can execute tasks. That is why we need to identify a method that can assist a real-time scheduler to determine when it would be optimal to go for charging the capacitor by analyzing training data.

In order to achieve this goal, we divide the audio signal that needs to be classified into blocks of audio segment where each block has a length of $t_{block}$ seconds. After sensing audio for $t_{block}$ seconds, we need to determine via a scheduling method when it would be most optimal to sense again in real-time. However if the execution algorithms consumes more energy than sensing continuously, it defeats the purpose of scheduling. That is why we decided to couple the scheduling algorithm with the classification algorithm. However since the scheduling should be done after sensing one block of audio signal, the classification algorithm should also be able to process data sequentially and not wait for the whole audio signal to be sensed.




==> tex/temp/05_sampler.tex <==

\section{Audio Sampler} 
In this section, we describe the process of classifying an audio event that has a length more than what an intermittent system can process continuously without power failure.

\subsection{Modeling Sensing Task}
SoundSieve considers the sensing and processing of a sensor data of longer duration for a classification task as a scheduling problem where it is not possible to complete all the jobs. We parameterize the scheduling problem as $\tau = (T_i, B_i, C_i)$, where $T_i$ represents the total length of the audio event that is to be classified, $B_i$ denotes the maximum number of audio blocks (chunks of audio with a fixed length) the intermittent system can process without completely exhausting the energy buffer, and $C_i$ denotes the ratio between the time needed to charge the energy buffer to process one block of audio and the time needed to discharge the energy buffer to process one audio block. If $C_i=1$, it means that the time needed to charge the energy buffer to process 1 block of audio is exactly the same as the time needed to discharge.

In general the value of $T_i$ and $B_i$ remains fixed throughout a certain intermittent sensing system, since the length of the audio event of a task and the processing cost for one block of audio remains fixed. However the value of $C_i$ can change at runtime depending on the energy harvesting rate.

\subsection{Scheduled Sampling}
After the sensor in SoundSieve wakes up due to an external event, the system transitions from low-power mode to active mode. Then the system reads and processes audio of a fixed window length, $t_{block}$. This processed audio is then fed into the RNN layer as mentioned in previous section and the final hidden state is saved in the system. Next, the system utilizes the importance predictor to estimate the importance of the next $n$ blocks in terms of classifying the audio event. Thus the problem becomes somewhat similar to priority scheduling problem.

However since the jobs here are sensing event, once the window has passed, there is no way to sense at that time point again. Hence, selecting the most important block does not make sense. Furthermore there is a possibility that deciding to sense according to the importance of each block may lead into the system fully charged but not in active sensing node. So the sampling scheduler needs to consider these scenario.

After we get the importance of next $n$ blocks, we consider sensing those blocks as jobs that need to be scheduled. If job, $J_i$ corresponds to sensing the audio block starting at time $t_i$, that means the job arrives at time $t_i$ and the deadline to complete this job is $t_i + t_{block}$. Since the execution time to sense and process this block is also $t_{block}$, the system has to either spend time and energy to complete this job, or conserve energy to wait for a job with higher priority. 

We first discard any jobs that have a negative negative, since negative value of importance of a time block corresponds to negative correlation with accuracy of the classification. After that we sort them according to the importance value. Suppose that sensing the block at time $t_i$ is most positively correlated to classify the signal. Then we calculate the amount of time the system waits with full energy if the sensing system is moved to low-power mode until time $t_i$. We use a threshold of such wait time $t_{idle}$ to determine if the system should until this time-step or move to the next most important block. Thus we make sure that the system does not spend any time waiting with full energy. We also estimate how much energy is left at this current time step. We chose a less important block of audio if the energy is lower than a threshold, to prepare the system to process more important block in the future. Thus we decide at which time step the system should start sensing again depending on the available energy and importance of each audio block.

After jumping to the next time point, the system does the same process again, until the whole audio is finished processing. This leaves us with a perforated audio, however since the perforation introduced here is not periodic and according to historical importance of each time point in a time-series data, the classification performance become better. A brief algorithm of the process is given in~\ref{algo:scheduling}.

Note that the idle time calculation depends on the energy harvesting rate which can change during run time. After the sound event is completed and there is no more audio block to process, the system starts classifying from the process audio blocks using the trained classifier.

\begin{algorithm}
\caption{Scheduling Audio Sampling}
\label{algo:scheduling}
\begin{algorithmic}[1]
\Require Block importance predictor $IP$, Audio classifier $f$, Charge and discharge ration $C_i$

\State $states_{rnn} = \{\}$
\While{$x\gets SenseAudio()$}
    \State $feature\gets Process(x)$
    \State $hidden\gets rnn(x, states_{rnn}[-1])$
    \State $states_{rnn}\gets states_{rnn}\cup hidden$
    \State $importance\gets IP(hidden, t_{current})$
    \State $importance\gets sort(importance)$
    \For{$t_{imp}\in importance$}
        \State $t_{idle}\gets CalculateWaitTime(imp, C_i, energy)$
        \If $t_{idle} > t_{threshIdle}$ 
        \State continue
        \EndIf
        \State break
    \EndFor
    \State $WaitUntil(t_{imp})$
\EndWhile
\State $y = f(hidden)$
\newline
\Return y
\end{algorithmic}
\end{algorithm}




==> tex/temp/algo.tex <==
After we get the importance of next $n$ blocks, we consider sensing those blocks as jobs that need to be scheduled. If job, $J_i$ corresponds to sensing the audio block starting at time $t_i$, that means the job arrives at time $t_i$ and the deadline to complete this job is $t_i + t_{block}$. Since the execution time to sense and process this block is also $t_{block}$, the system has to either spend time and energy to complete this job, or conserve energy to wait for a job with higher priority. 

We first discard any jobs that have a negative importance score, since negative importance score of a time block corresponds to negative correlation with accuracy of the classification. After that we sort them according to the importance value. Suppose that sensing the block at time $t_i$ is most positively correlated to classify the signal. Then we calculate the amount of time the system waits with full energy if the sensing system is moved to low-power mode until time $t_i$. We use a threshold of such wait time $t_{idle}$ to determine if the system should wait until this time-step or move to the next most important block. Thus we make sure that the system does not spend any time waiting with full energy. We also estimate how much energy is left at this current time step. We chose a less important block of audio if the energy is lower than a threshold, to prepare the system to process more important blocks in the future. Thus we decide at which time step the system should start sensing again depending on the available energy and importance of each audio block.

After jumping to the next block, the system does the same process again, until the whole audio is finished processing. This leaves us with a perforated audio, however since the perforation introduced here is not periodic and according to historical importance of each time point in a time-series data, the classification performance becomes better. A brief algorithm of the process is given in~\ref{algo:scheduling}.

Note that the idle time calculation depends on the energy harvesting rate which can change during run time. After the sound event is completed and there is no more audio block to process, the system starts classifying from the processed audio blocks using the trained classifier network.

\begin{algorithm}
\caption{Audio Sampler and Classifier}
\label{algo:scheduling}
\begin{algorithmic}[1]
\Require Block importance predictor $IP$, Audio classifier $f$, Charge and discharge ration $C_i$

\While{$x\gets SenseAudio()$}
    \State $feature\gets Process(x)$
    \State $importance\gets IP(feature, t_{current})$
    \State $importance\gets sort(importance)$
    \For{$t_{imp}\in importance$}
        \State $t_{idle}\gets CalculateWaitTime(imp, C_i, energy)$
        \If $t_{idle} > t_{threshIdle}$ 
        \State continue
        \EndIf
        \State break
    \EndFor
    \State $WaitUntil(t_{imp})$
\EndWhile
\State $y = f(hidden)$
\newline
\Return y
\end{algorithmic}
\end{algorithm}

==> tex/temp/features.tex <==
We use three widely-used frequency domain features to model the audio signal of block $t$. The first one is band energy ratio, which is calculated using the equation~\ref{eq3}.

\begin{equation}
    BER_t = \frac{\sum_{n=1}^{F-1} m_t(n)^2}{\sum_{n=F}^{N} m_t(n)^2}
    \label{eq3}
\end{equation}

This feature computes the ratio of the lower frequency components to the higher frequency components. We use $512$ Hz and $2048$ Hz as cutoff frequency for speech commands and audio events classification respectively.

The next feature we extract is the spectral centroid, which is the weighted mean of the frequency bins and can be computed using equation~\ref{eq4}.

\begin{equation}
    SC_t = \frac{\sum_{n=1}^{N} m_t(n)\times n}{\sum_{n=1}^{N} m_t(n)}
    \label{eq4}
\end{equation}

The final frequency domain feature we use is the spectral bandwidth which is the weighted mean of the distances of the frequency bins from the spectral centroid and can be computed using equation~\ref{eq5}.

\begin{equation}
    SC_t = \frac{\sum_{n=1}^{N} m_t(n)\times |n-SC_t|}{\sum_{n=1}^{N} m_t(n)}
    \label{eq5}
\end{equation}

We also add the current block number as an input and then feed them to a hidden FC layer followed by a output layer with $n$ outputs, where each output represents the predicted importance of a block. In this way, we formulate a simple and lightweight regression problem that can work as an audio sampler in real-world intermittent systems.
